The Many-Worlds Calculus

In this paper, we explore the interaction between two monoidal structures: a multiplicative one, for the encoding of pairing, and an additive one, for the encoding of choice. We propose a colored PROP to model computation in this framework, where the choice is parameterized by an algebraic side effect: the model can support regular tests, probabilistic and non-deterministic branching, as well as quantum branching, i.e. superposition. The graphical language comes equipped with a denotational semantics based on linear applications, and an equational theory. We prove the language to be universal, and the equational theory to be complete with respect to this semantics.

==> LMCS_-_submit/macros.tex <==
\def\mathunderline#1#2{\color{#1}\underline{{\color{black}#2}}\color{black}}
\def\rddots{.^{.^{.}}}

\newcommand{\one}{\ensuremath{\mathds{1}}}
\DeclareMathAlphabet{\mymathbb}{U}{BOONDOX-ds}{m}{n}
\newcommand{\zero}{\ensuremath{\mymathbb{0}}}

\newcommand{\inl}[1]{\ensuremath{\mathtt{inj}_l{\;#1}}}
\newcommand{\inr}[1]{\ensuremath{\mathtt{inj}_r{\;#1}}}
\newcommand{\pv}[2]{\ensuremath{\langle #1,#2 \rangle}}
\newcommand{\subf}[2]{\ensuremath{#1 \prec #2}}
\newcommand{\set}[1]{\ensuremath{\{#1\}}}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\posr}{\ensuremath{\mathcal{P}}}
\newcommand{\negr}{\ensuremath{\mathcal{N}}}
\newcommand{\ps}{\ensuremath{\mathcal{P_S}}}
\newcommand{\os}{\ensuremath{\mathcal{O_S}}}
\newcommand{\bs}{\ensuremath{\mathcal{B_S}}}

\newsavebox\MBox
\newcommand\Cline[2][red]{{\sbox\MBox{$#2$}%
  \rlap{\usebox\MBox}\color{#1}\rule[-1\dp\MBox-2pt]{\wd\MBox}{0.5pt}}}

\newcommand{\subst}[1]{\{\!| #1 |\!\}}
\newcommand{\rleadsto}{\mathbin{\reflectbox{$\leadsto$}}}
\newcommand{\rleadstos}{\mathbin{\reflectbox{$\leadsto^*$}}}
\newcommand{\alphaeq}{\approx_\alpha}
\newcommand{\polar}{\perp}
\newcommand{\cut}{\ensuremath{\mathtt{cut}}}
\newcommand{\exec}{\ensuremath{\mathtt{Ex}}}
\newcommand{\sol}{\ensuremath{\mathtt{Sol}}}

\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}

\usetikzlibrary{decorations.markings,arrows,decorations.pathmorphing, decorations.pathreplacing}
\usetikzlibrary{shapes.misc,matrix,backgrounds,folding,positioning}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{shapes.multipart}
\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{background,edgelayer,nodelayer,main}

\tikzset{every path/.style={draw=black!80, line width=0.6pt}}
\tikzstyle{every picture}=[baseline=-0.25em]
\tikzstyle{none}=[inner sep=0mm]
\tikzstyle{box}=[fill=white, draw=black, shape=rectangle]
\tikzstyle{zxnode}=[shape=circle, minimum width=.25cm, inner sep=0.5pt, font=\footnotesize, draw=black,thick]
\tikzstyle{gn}=[zxnode ,fill=green, draw=green!10!black]
\tikzstyle{rn}=[zxnode ,fill=red, draw=red!10!black]
\tikzstyle{H box}=[rectangle,fill=yellow, draw=yellow!10!black,thick,xscale=1,yscale=1,font=\footnotesize,inner sep=1.2pt,minimum width=0.15cm,minimum height=0.15cm]
\tikzstyle{ug}=[regular polygon, regular polygon sides=3, fill=red,draw=black,inner sep = 0pt,minimum width=0.8em]
\tikzstyle{black dot}=[inner sep=0.4mm,minimum width=0pt,minimum height=0pt,fill=black,draw=black,shape=circle]
\tikzstyle{dot}=[black dot]
\tikzstyle{white dot}=[dot,fill=white, inner sep=-1pt, font=\footnotesize]
\tikzstyle{arrow}=[decoration={markings,mark=at position 1 with
    {\arrow[scale=1.2,>=stealth]{>}}},postaction={decorate}]
\newcommand{\edgetick}{{\arrow[black,scale=0.7,very thick]{|}}}
\tikzstyle{glabel}=[rounded corners=0.2em,fill=green!30,inner sep=0.1em,font=\scriptsize, anchor=west, xshift=-0.3em, yshift=0,opacity=1]
\tikzstyle{rlabel}=[rounded corners=0.2em,fill=red!30,inner sep=0.1em,font=\scriptsize, anchor=west, xshift=-0.3em, yshift=0,opacity=1]
\tikzstyle{box}=[rectangle, draw=black, fill=white, inner sep=1pt, font=\scriptsize]
\tikzstyle{box-no-outline}=[rectangle, draw=white, fill=white, inner sep=2pt]
\tikzstyle{circle-no-outline}=[circle, draw=white, fill=white, inner sep=0pt]
\tikzstyle{squigglearrow}=[->, line join=round, decorate, decoration={zigzag, segment length=4, amplitude=0.8, post=lineto, post length=2pt}]
\tikzstyle{divide}=[regular polygon, regular polygon sides=3, draw=black, fill=gray!50, inner sep=1.6pt, rounded corners=0.8mm]
\tikzstyle{very thick}=[-, line width=1pt]
\tikzstyle{boxedge}=[draw=gray!50]
\tikzstyle{pbs}=[diamond, draw=black, inner sep=-0.5pt, fill=white]
\tikzstyle{ribbon}=[thick, rounded corners=0.4pt,fill={rgb,255: red,157; green,246; blue,255}, fill opacity=0.7]
\tikzset{tensor/.style={inner sep=2.5pt, draw=.!70!white, fill=.!70!white, circle, path picture={
			\draw[white]
			(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);
}}}
\tikzset{plus/.style={inner sep=2.5pt, draw, circle, path picture={
  \draw[black]
(path picture bounding box.east) -- (path picture bounding box.west) (path picture bounding box.south) -- (path picture bounding box.north);
}}}
\tikzstyle{contraction}=[circle,draw,font={\scriptsize \color{gray} c}, inner sep= 1pt]
\tikzstyle{small-contraction}=[circle,draw,font={\tiny  \color{gray} c}, inner sep= 0.2pt]
\tikzstyle{vacuum}=[rounded rectangle, draw, fill=gray!50, rounded rectangle west arc=none, rotate=180]
\tikzstyle{compact dash}=[dash pattern={on 2pt off 1pt}]

\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{background,edgelayer,nodelayer,main}

\tikzstyle{every loop}=[]

\usetikzlibrary{circuits.ee.IEC}

\colorlet{tapeBg}{red!30}
\colorlet{tapeBorder}{red!60}
\tikzstyle{tapeFill} = [fill=tapeBg]
\tikzstyle{tapeNoFill} = [draw=tapeBorder, line width=0.5pt]
\tikzstyle{tape} = [fill=tapeBg, draw=tapeBorder, line width=0.5pt]

\newcommand{\ground}
{
\begin{tikzpicture}[circuit ee IEC,yscale=0.9,xscale=0.8]
\draw[solid,arrows=-] (0,1ex) to (0,0) node[anchor=center,ground,rotate=-90,xshift=.66ex] {};
\end{tikzpicture}}

\newcommand{\sground}{\hspace*{-1pt}\scalebox{0.5}{\ground}}

\newcommand{\diode}
{
\begin{tikzpicture}[scale=0.1]
\filldraw[fill=white, draw=black] (0,-1) -- (-1.15,1) -- (1.15,1) -- cycle;
\draw (-1.15,-1) -- (1.15,-1);
\end{tikzpicture}
}

\newcommand{\tikzfig}[1]{
\InputIfFileExists{./figures/#1.tikz}{}{{\color{red}\colorbox{pink}{missing file : #1}}}
}

\def\fig{}

\iftoggle{extern}{
	\usetikzlibrary{external}
	\tikzexternalize[prefix=tikzfigs/]

	\let\oldtikzfig\tikzfig
	\renewcommand{\tikzfig}[1]{
		\tikzsetnextfilename{#1}
		\oldtikzfig{#1}}

	\newcommand{\tikzfigc}[1]{
		\tikzsetnextfilename{\fig_#1}
		\InputIfFileExists{./figures/\fig/\fig_#1.tikz}{}{{\color{red}\colorbox{pink}{missing file : #1}}}}
}{
	\newcommand{\tikzfigc}[1]{\InputIfFileExists{./figures/\fig/\fig_#1.tikz}{}{{\color{red}\colorbox{pink}{missing file : #1}}}}
}

\newcommand{\ket}[1]{\ensuremath{\left|  #1 \right\rangle}}
\newcommand{\bra}[1]{\ensuremath{\left\langle  #1 \right|}}
\newcommand{\ketbra}[2]{\ket{#1}\!\!\bra{#2}}
\newcommand{\braket}[2]{\left\langle\begin{array}{@{}c@{~}|@{~}c@{}} #1 & #2 \end{array}\right\rangle}
\newcommand{\tr}{\operatorname{Tr}}
\newcommand{\dom}{\operatorname{dom}}

\newcommand{\cat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\catD}{\ensuremath{\cat{C_D}}}
\newcommand{\interp}[1] {\left\llbracket #1 \right\rrbracket}
\newcommand{\ccpm}[1]{\operatorname{CPM}\left(#1\right)}

\newcommand{\rewrites}{\leadsto}

\newcommand{\sop}{\ensuremath{\rewrites_{\mathbf{sop}}}}

\newcommand{\cpm}{\ensuremath{\rewrites_{\sground}}}

\newcommand{\setirwer}{\rotatebox[origin=c]{180}{$\rewrites$}}

\newcommand{\downrewrites}{\rotatebox[origin=c]{-90}{$\rewrites$}}
\newcommand{\uprewrites}{\rotatebox[origin=c]{90}{$\rewrites$}}
\newcommand{\nerewrites}{\rotatebox[origin=c]{45}{$\rewrites$}}
\newcommand{\serewrites}{\rotatebox[origin=c]{-45}{$\rewrites$}}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}



\usetikzlibrary{cd}

\let\boxempty\relax
\DeclareMathOperator*{\boxempty}{\parallel}
\newcommand{\Implicit}[1]{\textbf{\textup{MW}}_{#1}}
\newcommand{\Explicit}[1]{\textbf{\textup{EMW}}_{#1}}
\newcommand{\FixedExplicit}[2]{\textbf{\textup{MW}}_{#2}}
\newcommand{\ManyWorlds}[1]{\textbf{\textup{MW}}_{#1}}
\newcommand{\oc}{\text{\textcircled{\textbf{c}}}}
\newcommand{\oscalar}[1]{\text{\textcircled{#1}}}
\newcommand{\oone}{\text{\raisebox{.5pt}{\textcircled{\raisebox{-.9pt}{\textbf{1}}}}}}
\newcommand{\ozero}{\text{\raisebox{.6pt}{\textcircled{\raisebox{-1.0pt}{\textbf{0}}}}}}
\newcommand{\bfup}[1]{\textup{\textbf{#1}}}
\newcommand{\id}{\textup{\textbf{id}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Mat}{\mathcal{M}}
\newcommand{\FdM}{\mathbf{FdS}_R}
\newcommand{\withWorld}[2]{{#1}_{\scaleto{#2}{4pt}}}

\newcommand{\emptysquare}{\ensuremath{\varnothing}}
\newcommand\goth[1]{\textgoth{#1}}
\newcommand\ngoth[1]{\textgoth{#1}}

\DeclareMathOperator{\tensor}{
\text{\scalerel*{%
		\iftoggle{extern}{\tikzsetnextfilename{tensor}}{}
		\begin{tikzpicture}
		\node[inner sep=2pt, draw=.!70!white, circle, fill=.!70!white, path picture={
			\draw[white]
			(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east);
		}] (c) at (0,0){};
		\end{tikzpicture}}{\otimes}}}

\DeclareMathOperator{\contraction}{
\scalerel*{%
		\iftoggle{extern}{\tikzsetnextfilename{contraction}}{}
		\begin{tikzpicture}
		\node[inner sep=2pt, draw=., circle, font={c}] (c) at (0,0){};
		\end{tikzpicture}}{\oplus}}

\newcommand{\iso}{\operatorname{iso}}
\newcommand{\inv}{\text-\scalebox{0.7}{$1$}}

\newcommand{\enab}[1]{#1^\bullet}
\newcommand{\enabW}[2]{{#1}\cap #2}

\renewcommand{\aa}{\textcolor{black!50!green}{a}}
\newcommand{\bb}{\textcolor{red}{b}}
\newcommand{\xx}{\textcolor{violet}{x}}
\newcommand{\cblue}{\textcolor{blue}{c}}
\newcommand{\sstar}{\textcolor{gray}{\star}}

\makeatletter\setlength\BA@colsep{5pt}\makeatother

\newcommand{\alt}{~\mid~}
\newcommand{\bor}{\alt}
\newcommand{\isot}{\leftrightarrow}
\newcommand{\defeq}{\stackrel{\vartriangle}{=}}
\newcommand{\pp}{+\!\!\!+}
\newcommand{\arrowp}[2]{ #1 \;+\!\!\!+\; #2}
\newcommand{\bind}{\mathbin{>\!\!\!>\mkern-6.7mu=}}
\newcommand{\foldv}[1]{\langle #1 \rangle}
\newcommand{\letpv}[3]{{\tt let}\,{\langle #1 \rangle}={#2}~{\tt in}~{#3}}
\newcommand{\letv}[3]{{\tt let}\,{#1}={#2}~{\tt in}~{#3}}
\newcommand{\isobasique}{\ensuremath{\{v_1~\isot~e_1 \alt \dots \alt v_n~\isot~e_n\}}}
\newcommand{\tc}{\mathtt{t}\!\mathtt{t}}
\newcommand{\fc}{\mathtt{f}\!\mathtt{f}}
\newcommand{\isoterm}{\omega}
\newcommand{\isoneg}{\ensuremath{\omega^{-1}}}
\newcommand{\entailval}{\vdash_v}
\newcommand{\entailiso}{\vdash_{\isoterm}}
\newcommand{\entailterm}{\vdash}
\newcommand{\scalprod}[2]{\langle#1|#2\rangle}
\newcommand{\opn}[1]{\ensuremath{\operatorname{#1}}}
\DeclarePairedDelimiter\pparenthesis{\llparenthesis}{\rrparenthesis}

